Algorithm for Optimized mRNA Design Improves Stability and Immunogenicity

Messenger RNA (mRNA) vaccines are being used for COVID-19, but still suffer from the critical issue of mRNA instability and degradation, which is a major obstacle in the storage, distribution, and efficacy of the vaccine. Previous work showed that optimizing secondary structure stability lengthens mRNA half-life, which, together with optimal codons, increases protein expression. Therefore, a principled mRNA design algorithm must optimize both structural stability and codon usage to improve mRNA efficiency. However, due to synonymous codons, the mRNA design space is prohibitively large, e.g., there are $\sim\!10^{632}$ mRNAs for the SARS-CoV-2 Spike protein, which poses insurmountable challenges to previous methods. Here we provide a surprisingly simple solution to this hard problem by reducing it to a classical problem in computational linguistics, where finding the optimal mRNA is akin to finding the most likely sentence among similar sounding alternatives. Our algorithm, named LinearDesign, takes only 11 minutes for the Spike protein, and can jointly optimize stability and codon usage. Experimentally, without chemical modification, our designs substantially improve mRNA half-life and protein expression in vitro, and dramatically increase antibody response by up to 23$\times$ in vivo, compared to the codon-optimized benchmark. Our work enables the exploration of highly stable and efficient designs that are previously unreachable and is a timely tool not only for vaccines but also for mRNA medicine encoding all therapeutic proteins (e.g., monoclonal antibodies and anti-cancer drugs).

==> Makefile <==
texbin=/Library/TeX/texbin
#texbin=/usr/local/texlive/2018/bin/x86_64-darwin
main:
	rm -rf *.run.xml *.bcf *.aux *.out *.blg *.bbl *.log *.fls *.fdb_latexmk *~
	${texbin}/pdflatex main
	${texbin}/bibtex main
	if ${texbin}/bibtex siref; then \
		echo "seperate references\n"; \
	else \
		echo "combined references\n"; \
	fi
	${texbin}/pdflatex main
	${texbin}/pdflatex main

split:
	yes | gs -dBATCH -sOutputFile="main.submit.pdf" -dFirstPage=1 -dLastPage=18 -sDEVICE=pdfwrite main.pdf 
	yes | gs -dBATCH -sOutputFile="supp.pdf" -dFirstPage=19 -sDEVICE=pdfwrite main.pdf  

clean:
	rm -rf  *.run.xml *.bcf *.xwm *.aux *.out *.blg *.log *.fls *.fdb_latexmk main.pdf *~ 

fast:
	${texbin}/pdflatex main


==> result_insilico.tex <==
% !TEX root = main.tex

% \subsection*{Search Quality of Linear-time Approximation}

\iffalse
\paragraph{Approximation Quality of Beam Search}

% Since the \lineardesign algorithm is significantly faster than its exact counterpart, 
% we envision that the \lineardesign algorithm will be used for long sequences. 
To ensure the quality of the approximation used in \lineardesign (with beam pruning mode), 
we investigate the search error between the exact and approximate algorithm ($b = 500$ and $b = 100$).
 % in Fig.~\ref{fig:insilico}B and C. 
% For this analysis, we used the same dataset as in subsection~\ref{sec:result}\ref{subsec:runtime}.
% Fig.~\ref{fig:insilico}B and C represent the search error between the exact mode and the approximate mode.
% In Fig.~\ref{fig:insilico}B, 
% we compare the free energy changes of the mRNA sequences designed with exact search and with the $b=1,000$ approximation. 
% The x-axis is the free energy of exact search,
% while the y-axis corresponds to the free energy of approximation.
% We see that all plots are on or close to the diagonal,
% which confirms that the folding free energy differences are 0 or small. 
% We show that the free energy gaps, 
% which are the differences of the free energy change between two modes ($\Delta \Delta G^{\circ} = \Delta G^{\circ}_{\mathrm {appr.}} - \Delta G^{\circ}_{\mathrm {exact}}$) divided by the MFE of the sequence designed by exact mode ($\Delta G^{\circ}_{\mathrm {exact}}$), are small when only optimizing the MFE.
Regarding free energy gaps in Fig.~\ref{fig:insilico}B, for $b=500$ all sequences have gaps within 2.5\%, 
e.g., the gaps of the \spike coding region (3,822~\nts) and the longest sequence (9,999~$nt$ including stop codon) are 1.2\% and 1.5\%, respectively.
For a smaller beam size $b=100$, the gaps are all within 6\% except for three sequences (within 7.5\%), 
and specifically, the gaps of the \spike gene and the longest sequence are 3.6\% and 4.8\%, respectively.
% For $b=100$, most gaps are within 5\%, and the largest gap is at around 7\%.
Similarly, Fig.~\ref{fig:insilico}C compares the gap of MFE-CAI joint optimization on the mRNA sequence that encodes \sarscovtwo \spike protein.
% Here the gap is defined as
% $(\Delta \Delta G^{\circ} + \lambda \Delta \mathrm{CAI}) \ / \ (\Delta G^{\circ}_{\mathrm {exact}} + \lambda \mathrm{CAI}_{\mathrm {exact}})$,
% where $\mathrm{CAI}_{\mathrm {exact}}$ is the \CAI of the sequence designed by exact mode, 
% $\Delta \mathrm{CAI}$ is the \CAI difference of two sequences from two modes, respectively,
% and $\lambda$ is a hyperparameter balancing \MFE and \CAI.
We observe that the gaps are small, 
all within 1.5\% for $b=500$,
and all within 5.5\% for $b=100$,
and go down to zero quickly with the increase of $\lambda$ for $b=500$.    
Additional correlations between search error and sequence length are shown in Fig.~\ref{fig:breakdown_gap}. 

\fi
% trend of free energy differences increases linearly with mRNA sequence length.
% They y-axis is the percentage of free energy change gap,
% which is the free energy change gap ($\Delta \Delta G^{\circ}$) divided by the total free energy change of the MFE structure ($\Delta G^{\circ}$). 
% The percentage of free energy change gap is small for all sequences in the dataset.
% For $b=1,000$, all sequences have gaps within 1\%. 
% Even for the longest sequence (8,484~$nt$), the gap is 0.8\%.
% For $b=100$, most gaps are within 5\%, 
% and the largest gap is 7\%.
%We also investigate the percentage of free energy change gap against beam size for the spike protein of SARS-CoV-2
%% two specific protein sequences, the spike protein of SARS-CoV-2 and EGFP (GenBank KM042177.1),
%in Fig.~\ref{fig:local_mode_compare}A,
%which comfirms that the search error of \lineardesign decrease quickly with the increase of beam size,
%and compare the search error between CDSfold (local mode) and \lineardesign (beam search mode) in Fig.~\ref{fig:local_mode_compare}B,
%which shows that \lineardesign runs much faster than CDSfold for a similar search error level.
%In Fig.~\ref{fig:local_mode_compare}C--E, secondary structures of sequences designed by CDSfold and \lineardesign are shown as example,
%illustrating that the structures of \lineardesign sequences are globally optimized.
%% More interesting, studies show that the 5’ and 3’ end distances of long RNAs (1,000 to 10,000nt) are always in few nanometers (Lai et al., 2018) (3nm in average (Yoffe et al., 2011)). 
%We test the end-to-end (ETE) distance of the three designs using RNAstructure~\cite{reuter2010rnastructure},
%and find the ETE distances of \lineardesign are smaller and more in line with previous study~\cite{lai+:2018}.
% The ETE distance is 9.05nm of CDSfold with w = 500, while for b = 300 and b = 600 LinearDesign designs, the ETE distances are
% 3.14nm and 1.77nm respectively.
% Starting with a small beam size, $b=100$, the gap is 3.53\%. 
% With increasing beam size, the gap shrinks quickly to 1.21\% at $b=500$. 
% Further increasing beam size up to 900, the gap drops to 0.55\%. 
% With a beam size of $b=1,500$ the gap drops to 0.25\%. 
% This happens because more states are kept when enlarging the beam size, among which states with higher scores at length j survive.


% \subsection*{Species-specific Correlation Between \MFE and \CAI}
% \subsection*{Example for the mRNA Coding Region of SARS-CoV-2 Spike Protein}

\iffalse
\paragraph{Case Study: mRNA for \sarscovtwo \spike Protein}

% Fig. 3D 3E
% It is well-known that codon usage is different across species,
% e.g., GC-rich codons are favored by mammals, 
% while AU-rich codons are more frequent in \textit {\ecoli}~\cite{chamary2006hearing,maloy1996genetic,grantham1980codon}.
% This codon bias leads to species-specific correlation between \MFE and \CAI.
% Since GC pair is stronger than AU pair,
% optimizing \CAI results in more GC-rich codons, 
% which decreases \MFE for mammals but increases \MFE for \ecoli.
% % Fig.~\ref{subsec:insilico}D and E show that this correlation is partially true.
% This correlation is partially confirmed by our \insilico computation,
% yet becomes invalid when approaching to the boundary of the design space.
In Fig.~\ref{fig:insilico}B, % is a two-dimensional (MFE--CAI) illustration 
%of the mRNA design space  
%represents the \MFE and \CAI of different 
%the mRNA candidates 
%for the \sarscovtwo \spike protein. % in the style of Fig.~\ref{fig:overview}C.
%with \MFE on the $x$-axis (the lower the better) and \CAI (calculated using the human codon table)
%on the $y$-axis (the higher the better).
the wildtype\footnote{From the \sarscovtwo reference sequence: https://www.ncbi.nlm.nih.gov/nuccore/MN908947.} (red circle)
has rather non-optimal CAI and MFE. %of 0.655 and an MFE of 
%folds into an modestly stable structure of MFE  %-1075.40~kcal/mol,
%change of 
%-$967.80$~kcal/mol 
%and has a CAI of 0.655 
%(the red circle).
%Additionally, 
%As baselines, 
We used two random search strategies, {\em uniform} and {\em codon-biased}, to generate %random sequences (
50,000 sequences each; they improved both MFE and CAI, but only slightly, due to just scratching %covering
a tiny fraction of the exponentially large search space. %combinatorial explosion.
%, they do not go very far. %) as point clouds. % as other baselines.
% The first strategy, named ``uniform random'', is to randomly (with equal probabilities) choose a codon for each amino acid (the dark-blue cloud); 
% the ``codon-biased random'' strategy 
% is to choose a codon with the probability proportional to its usage frequency (the orange cloud).
% and the last one is ``codon-biased random with sharp peak'', 
% whose codons are generated with a more peaked usage frequency distribution (the light-blue cloud).
%On the top-right is the optimal-CAI design by always choosing 
%the most frequent codon for each amino acid (the Gray circle).
%Finally, the CAI-greedy design (the Gray dot) is to select the most frequent codon for each amino acid,
%which has a \CAI of 1.
As human genes prefer GC-rich codons,\footnote{the human and yeast codon usage frequencies are from {\scriptsize \myurl{https://www.genscript.com/tools/codon-frequency-table}.}}
optimizing \CAI
via codon optimization (the arrow)
%It clearly shows that with optimizing \CAI, 
also improves \MFE, by about 400 kcal/mol from the wildtype to the optimal-CAI design. %from about $-1,000$ kcal/mol to about $-1,400$ kcal/mol
%(``codon optimization'' arrow).
%In fact, codon optimization is the standard method of  mRNA design, 
%used by the vaccines of BioNTech-Pfizer and Moderna. % are both optimized in codon choice as compared to wildtype.
%In fact, most designs of the vaccine companies are in the regions that close to CAI-greedy design.  
%We also visualized 
The light blue curve shows \lineardesign's optimal sequences %LinearDesign-optimized sequences 
%(varying $\lambda$), % are shown
%in 
between $\lambda\!=\!0$ (optimal MFE) and $\lambda\!=\!\infty$ (optimal CAI). % designs.
%being the optimal-MFE 
%and optimal-CAI designs, respectively.
%and $\lambda=\infty$ is the optimal-CAI design.
%on which the leftmost dot representing the sequence with the lowest \MFE globally.
Each point on this curve achieves %stands for a sequence with
the lowest \MFE for a given \CAI
(or the highest \CAI for a given \MFE),
making it the feasibility limit of all  $\sim2.4 \times 10^{632}$ designs.
%,
%beyond which no candidates exist. % to the upper-left side of this curve.
%beyond which no candidate sequence exist.
%i.e., no sequences can achieve the region beyond this curve.
%We can see that there is a huge territory to the left of the line $x=-1,400$ kcal/mol,
%because further optimizing \MFE beyond that is out of the reach of codon optimization,
%and requires efficient combinatorial optimization algorithms 
%like ours. %becomes harder and harder.
%When approaching  this design boundary, \MFE and \CAI become anti-correlated,
%meaning that 
%which means we 
%having to sacrifice one to optimize the other.
%Interestingly, If we extended the design boundary to the low \CAI direction, 
%we can see that it forms a half oval.
However, for the yeast codon preference (Fig.~\ref{fig:insilico}C),  
the \MFE and \CAI improvements are anti-correlated due to a bias for AU-rich codons,
and the design boundary moves lower-right. %rotates towards the left-bottom corner 
See  Fig.~\ref{fig:human_yeast_codon_oval_full} for negative $\lambda$'s.
% for
%the lower-left design boundaries with negative $\lambda$'s.
% additional results with negative $\lambda$'s (i.e., the lower-left design boundaries).
\fi




==> results.tex <==
% !TEX root = main.tex


The mRNA design problem can be formulated as follows:
given a protein sequence $\vecp=p_1 \ldots p_m$ where each $p_i$ is an amino acid, 
we search, among all possible mRNA sequences $\vecr$ that translate into  protein \vecp, the best mRNA sequence $\vecr^\star(\vecp)$, 
% whose minimum free energy is the lowest:
defined as the sequence that has the structure with minimum folding free energy change:

\vspace{-.5cm}\begin{equation*}
\begin{split}
 \vecr^\star(\vecp) & = \argmin_{\vecr \in \RNA(\vecp)} \MFE(\vecr) \\
 \MFE(\vecr) & = \min_{\vecs \in \structures(\vecr)} \freeenergy(\vecr, \vecs)
\end{split}
\end{equation*}
where  $\RNA(\vecp) = \{ \vecr \mid \protein(\vecr) = \vecp \}$ is the search space,
$\structures(\vecr)$ is the set of all possible secondary structure for RNA sequence \vecr,
and $\freeenergy(\vecr, \vecs)$ is the free energy change of structure~\vecs for RNA~\vecr according to an energy model.

Since codon usage is important for mRNA translation efficiency and functional half life~\cite{mauger+:2019}, it is better to consider jointly optimizing mRNA stability 
% (measured by the minimum folding free energy, i.e., \MFE) 
and codon usage. 
% (measured by codon addaptation index, i.e., \CAI). 
Therefore, \CAI can be integrated as an additive regularization term in the objective function:
\begin{equation*}
\begin{split}
% \vecr^\star(\vecp) & = \argmin_{\vecr \in \RNA(\vecp)} \MFE(\vecr) \\
\vecr^\star(\vecp) & = \argmin_{\vecr \in \RNA(\vecp)}\Big({\MFE(\vecr)}- (m+1) \lambda \log {\CAI(\vecr)}\Big) \\
                   & = \argmin_{\vecr \in \RNA(\vecp)}\Big({\MFE(\vecr)}- (m+1) \lambda \log (\Pi_{i=1}^{m+1}w_i(\vecr))^{\frac{1}{m+1}}\Big) \\
                   & = \argmin_{\vecr \in \RNA(\vecp)}\Big({\MFE(\vecr)}- \lambda \sum_{i=1}^{m+1} {\log} w_i(\vecr)\Big)
\end{split}
\end{equation*}
where $m$ is the protein length, ${\log} w_i(\vecr)$ is the measurement of deviation from the optimal codon (0 is optimal) for the $i$th amino acid (given an mRNA candidate),
and $\lambda$ is a hyperparameter that balances \MFE and \CAI.

% We first introduce our mRNA sequence design algorithms
To solve the above mRNA sequence design problem, 
we develop efficient algorithms that can optimize folding stability, 
as well as optimize stability and protein expression jointly,
and further accelerate our algorithms with beam pruning technic.
We show that our algorithms are orders of magnitude faster than the baseline, 
and can design coding region of \sarscovtwo \spike protein in about 10 minutes.
Finally, we design several mRNA sequences encoding the \spike protein using our algorithms, 
and perform multiple assays to characterize these designs with a particular focus on
stability, expression, and immunogenicity. 
Our designs substantially improve \insolution chemical stability and \incell protein expression over the codon-optimized benchmark, 
and increase neutralizing antibody titration by up to $20\times$ \invivo. 

